Get Experience from Practice: LLM Agents with Record & Replay

AI agents, empowered by Large Language Models (LLMs) and communication protocols such as MCP and A2A, have rapidly evolved from simple chatbots to autonomous entities capable of executing complex, multi-step tasks, demonstrating great potential. However, the LLMs' inherent uncertainty and heavy computational resource requirements pose four significant challenges to the development of safe and efficient agents: reliability, privacy, cost and performance. Existing approaches, like model alignment, workflow constraints and on-device model deployment, can partially alleviate some issues but often with limitations, failing to fundamentally resolve these challenges. This paper proposes a new paradigm called AgentRR (Agent Record & Replay), which introduces the classical record-and-replay mechanism into AI agent frameworks. The core idea is to: 1. Record an agent's interaction trace with its environment and internal decision process during task execution, 2. Summarize this trace into a structured "experience" encapsulating the workflow and constraints, and 3. Replay these experiences in subsequent similar tasks to guide the agent's behavior. We detail a multi-level experience abstraction method and a check function mechanism in AgentRR: the former balances experience specificity and generality, while the latter serves as a trust anchor to ensure completeness and safety during replay. In addition, we explore multiple application modes of AgentRR, including user-recorded task demonstration, large-small model collaboration and privacy-aware agent execution, and envision an experience repository for sharing and reusing knowledge to further reduce deployment cost.

==> design-ebac.tex <==
\section{Design: Experience-Based Agent Execution (EBAE)}

We now detail the design of the Experience-Based Agent Execution (EBAE) framework, including the core Experience abstraction and the Record, Summary and Replay phases.

\subsection{Core Idea and Architecture}

The fundamental principle of EBAE is to ensure agent safety by constraining its procedural actions to align with observed human behavior.
It operates like "training wheels" for agents performing complex tasks: the agent is guided along paths previously traversed or approved by a human, preventing it from taking unexpected or potentially unsafe procedural detours.
A critical design choice is the separation between procedural execution and creative generation.

Procedural actions encompass the sequence of operations involving tool invocation, interaction with specific UI elements (clicks, typing in specific fields), navigation between applications, or API calls that constitute the workflow's structure.
In our conceptual model, these are the directed edges connecting states.
EBAE primarily constrains these actions.
Creative actions involve tasks where the agent leverages its core intelligence (typically an LLM) to generate content, make complex decisions, or perform actions within the confines of a specific tool or application state.
Examples include drafting email text, summarizing a document, generating code within an IDE, or selecting items based on complex criteria.
These correspond to the nodes or states in our conceptual model.
EBAE allows flexibility within these nodes, assuming the tool itself or other mechanisms (like LLM guardrails) provide safety for the creative generation itself.

The overall architecture revolves around the lifecycle of an "Experience".

\subsection{The Experience Abstraction}

An Experience is the central artifact in EBAE, representing a known-safe, potentially generalized workflow for accomplishing a specific task.
We propose representing an Experience as a directed graph, specifically a form of state machine.
Nodes represent significant, abstract states in the workflow or points where creative action is permitted.
A node might correspond to having a specific application open and focused (e.g., "Email Client Active," "Web Browser on Search Results Page") or reaching a logical milestone.
Creative actions are associated with nodes, allowing the agent to operate within the context defined by the node (e.g., use the LLM to generate text while the "Email Client Active" node is current).
State abstraction is crucial here to merge similar low-level system snapshots into meaningful abstract states.

Edges represent the procedural actions that transition the system between states.
These correspond to specific, observable operations like "Click `Send' Button," "Execute Search Query `X'," "Open File `Y'," "Call API `Z'."
These edges are the primary target of constraints during Replay.
Each edge is annotated with conditions or check functions necessary for enforcing Execution Flow Integrity (detailed in Section~\ref{sec:efi}).

An ideal Experience possesses several properties: verifiability, generalizability, and reusability.
The procedural flow defined by the Experience should be amenable to formal analysis or verification to provide strong safety guarantees.
An Experience should capture the essential logic of a task, allowing it to be replayed in slightly different contexts (e.g., with different input data) than the original recording(s).
Experiences should be sufficiently well-defined to be stored, shared, and reused for recurring tasks.

\subsection{Record Phase: Capturing User Traces}

The goal of the Record phase is to capture a faithful sequence of user actions performed across potentially multiple applications and tools while completing a task instance.
Accurately capturing actions across application boundaries is difficult.
Low-level events (mouse clicks, key presses) need to be mapped to semantically meaningful actions (e.g., "Click Save Button," "Type username").
Handling concurrent user actions or background processes can add noise.
The recording process must have minimal performance impact on the user's system.
Privacy is also a concern, as recordings might capture sensitive information.

\iffalse
A practical implementation likely requires a combination of techniques: UI Automation APIs, system-wide event hooking, and browser extensions.
Platforms like Windows UI Automation or macOS Accessibility APIs provide programmatic access to UI elements across many applications.
These can be used to identify the element being interacted with (button, text field) and the action (click, type).
Tools like Inspect.exe aid in exploring the UI tree.
Frameworks like Selenium, Playwright, etc., are powerful for web interactions.
Intercepting input events (mouse, keyboard) globally using OS-specific mechanisms (CGEventTap on macOS, SetWindowsHookEx on Windows) provides broad coverage but requires careful mapping of low-level events to high-level UI elements and actions, potentially using Accessibility APIs to get context at the time of the event.
API hooking can capture interactions at a different level.
While primarily for system calls and network traffic, eBPF could potentially capture system events triggered by UI actions or monitor process interactions resulting from user input, offering low overhead and good visibility.
It requires kernel support (primarily Linux).
For web-based parts of a task, browser extensions can capture detailed DOM events, user inputs, and network requests with high fidelity.
The Chrome DevTools Recorder provides a mechanism for recording and exporting user flows.
Techniques similar to distributed tracing context propagation or explicit user identification mechanisms (like Smartlook's Identify API) might be needed to link actions across different processes or platforms into a single task trace.
\fi

The output of the Record phase is a trace, typically a time-ordered sequence of events.
Each event should capture: timestamp, action type (e.g., click, type, keypress, tool\_call), target application/window, target UI element identifier (e.g., accessibility ID, XPath, CSS selector), action parameters (e.g., typed text, coordinates), and potentially a snapshot of relevant state variables.
Privacy-sensitive data might need to be masked or anonymized during recording or before storage.

\subsection{Summary Phase: Generalizing Traces to Experience}

This phase transforms one or more raw execution traces into a generalized, reusable Experience graph.
This is arguably the most challenging and critical phase for ensuring both utility and safety.
Traces for the same task may exhibit variations due to user choices, different starting states, or minor environmental changes.
The Summary process must identify the core workflow while abstracting away non-essential details (e.g., specific coordinates of a click on a button, exact text typed if it is input data).
Crucially, the generalization must not introduce unsafe behaviors; the resulting Experience must accurately reflect the safe operational boundaries demonstrated by the user(s).
This requires careful handling of abstraction and potentially integrating verification.

\iffalse
Potential techniques include process mining and program synthesis.
Process discovery algorithms can be applied to the sequence of semantic actions extracted from the trace(s).
Algorithms like Inductive Miner or Heuristics Miner can infer workflow structures (sequence, choice, parallelism, loops) from the event sequences.
Using techniques designed for UI logs or adopting hybrid model discovery might be necessary.
The output model forms the basis of the Experience graph.
Treating traces as demonstrations and synthesizing a workflow program is another approach.
Techniques could include learning regular expressions or automata from action sequences to capture control flow, using template-based synthesis where the user provides a high-level structure, and employing LLMs to help generalize or structure the workflow based on the trace and task description.
Crucially, synthesis must prioritize safety and verifiability.
The synthesized Experience should be in a form amenable to the checks performed during Replay.
Identifying similar states across traces or within a single trace and merging them into abstract nodes in the Experience graph requires defining state similarity metrics and ensuring the abstraction preserves safety-relevant distinctions.
Predicate abstraction or learning state invariants might be applicable.
Finding frequently occurring subsequences of actions across traces to identify core parts of the workflow is another technique.
\fi

Safety during generalization is paramount.
Simply merging paths or abstracting parameters can inadvertently create an Experience that allows unsafe sequences not present in the original traces.
Approaches to mitigate this include constrained generalization, verification-in-the-loop, user auditing, and parameter analysis.
Constrained generalization limits the types of generalizations allowed (e.g., only abstract data values, not control flow unless explicitly supported by multiple traces).
Verification-in-the-loop integrates formal verification techniques during or after generalization.
For example, checking if the generalized Experience satisfies safety properties derived from the original traces or predefined rules.
User auditing requires human review and approval for generalized Experiences before they are marked as safe in the Experience Store.
Parameter analysis involves analyzing how variable parameters affect safety.
Ensure that for any valid instantiation of variable parts within defined bounds, the workflow remains safe.
This might involve symbolic execution or abstract interpretation over the Experience graph.

\subsection{Replay Phase: Agent Execution and Audit}

During Replay, the agent executes the task guided by a chosen Experience (or a raw trace if no suitable Experience exists).
The agent conceptually traverses the Experience graph.
When encountering a procedural edge, the agent retrieves the associated action and parameters.
Before execution, the Execution Flow Integrity mechanism (Section 5) verifies the transition using check functions.
If approved, the agent executes the action (e.g., calls an application API, simulates a UI interaction).
If the edge involves generalized parameters, the agent may need to instantiate them based on the current runtime context (e.g., finding the current window handle, selecting the correct file based on a pattern).
When the agent reaches a creative node, control is temporarily passed to the agent's internal logic (e.g., LLM).
The agent performs its creative task within the context defined by the node (e.g., generating text in the currently focused editor).
Upon completion of the creative task, the agent signals readiness to proceed, potentially triggering the next procedural step based on the Experience graph.

As the procedural decision path is largely determined by the Experience, the cognitive load on the agent is reduced compared to figuring out the workflow from scratch.
This should ideally lead to faster and more efficient execution for the procedural parts of the task.

Throughout the Replay, a dedicated logger records every significant event: the Experience ID being used, each procedural action attempted, the outcome of the Integrity Check, the actual execution result (success/failure), and any significant events from creative nodes (e.g., content generated).
Timestamps are associated with all entries.
The audit log serves multiple purposes: debugging failed replays, providing evidence for compliance, enabling security forensics if the agent causes harm despite controls, and generally providing accountability by linking agent actions back to the specific Experience that guided them.
This aligns with the goals of system provenance.

\subsection{Experience Store}

The Experience Store acts as a central repository for managing Experiences.
It allows users to upload Experiences generated from their traces, download Experiences created by others, search for Experiences relevant to specific tasks, rate the quality and reliability of Experiences, and potentially mark Experiences as formally audited or verified.
The store is likely implemented as a database storing the Experience graphs (e.g., serialized as JSON or a graph database format) along with associated metadata (task description, creator, version, ratings, audit status, usage statistics).
It provides an interface for users or agents to query and select the most appropriate Experience for a given task based on criteria like task similarity, user ratings, success rate, or verification status.

\subsection{Ground Truth and Security Model}

The security of EBAE relies on the concept of "ground truth" derived from human actions.
A raw trace recorded directly from a user's actions is considered ground truth and inherently safe for that specific instance.
A generalized Experience is considered safe only if: (a) it was generated using a provably safe summarization technique, OR (b) it has been manually audited and approved by a trusted user, OR (c) it has passed automated verification checks against defined safety properties.
Users implicitly trust their own recorded actions.
Trust in shared Experiences from the store depends on the store's mechanisms for rating, verification, and potentially cryptographic signing or provenance tracking of the Experiences themselves.

\iffalse
\subsection{Experience Hierarchy and Abstraction}

To handle complexity and improve generalization, Experiences can be structured hierarchically.
Low-level Experiences might detail specific sequences of clicks and keystrokes.
Higher-level Experiences could abstract these sequences into semantic actions like "Login to System," "Generate Monthly Report," or "Submit Order."
An edge in a high-level Experience might correspond to an entire sub-Experience at a lower level.
Abstraction can make Experiences more robust to minor UI changes, easier for humans to understand and audit, and potentially allow for reuse of common sub-workflows across different tasks.
This hierarchy could be achieved through hierarchical process discovery algorithms during the Summary phase, manual composition of Experiences by users, and applying state abstraction techniques to group sequences of low-level actions into higher-level transitions.
\fi

==> design-efi.tex <==
\section{Execution Flow Integrity Enforcement}
\label{sec:efi}

Execution Flow Integrity (EFI) is the core mechanism ensuring that the agent adheres to the procedural constraints defined by a safe Experience during the Replay phase. It acts as a runtime reference monitor guided by the Experience.

\subsection{State Transition System Model}

We model the agent's interaction with the environment during replay as a State Transition System (STS).

\textbf{States (S):} A state represents a snapshot of the relevant aspects of the system environment at a given point in time. The definition of "state" is flexible and task-dependent. It could include: the currently focused application and window, the status or content of specific UI elements, relevant file system information, values of critical variables, or even abstract states derived from these (e.g., "Logged In," "File Open"). Effective state abstraction is crucial to define a manageable yet sufficiently expressive state space. Similar concrete states might be merged into abstract states corresponding to the nodes in the Experience graph.

\textbf{Actions (A):} Actions correspond to the procedural operations represented by the edges in the Experience graph. These are the transitions the agent attempts to execute, such as \texttt{click(button\_id)}, \texttt{type(text\_field\_id, 'text')}, \texttt{call\_api(endpoint, params)}.

\textbf{Transitions:} A transition $S \xrightarrow{A} S'$ denotes that executing action $A$ in state $S$ leads to state $S'$. The Experience graph defines the allowed transitions.

\textbf{Trajectories:} A complete execution of a task during replay corresponds to a trajectory through the STS, which is a sequence of states and actions: $S_0 \xrightarrow{A_1} S_1 \xrightarrow{A_2} S_2 \cdots \xrightarrow{A_n} S_n$. The goal of EFI is to ensure that this trajectory is valid according to the chosen Experience.

\subsection{Mapping Experience to the STS}

The Experience graph, learned during the Summary phase, serves as the specification for allowed trajectories.

Nodes in the Experience graph map to (potentially abstract) states or sets of states ($S$) in the STS.

Edges in the Experience graph define the allowed actions ($A$) and the valid transitions between these states. An edge from node $N_1$ to node $N_2$ labeled with action $A$ implies that action $A$ is permitted when the system is in a state corresponding to $N_1$, and its successful execution should lead to a state corresponding to $N_2$.

\subsection{Check Functions}

Before the Replayer executes any procedural action $A$ corresponding to an edge in the Experience graph, EFI invokes a set of check functions associated with that edge. These functions act as runtime guards or predicates, analogous to the checks performed by a reference monitor.

\textbf{Purpose:} To verify that executing action $A$ from the current state $S_{\text{current}}$ is permissible according to the Experience and known safety constraints.

\textbf{Derivation:} Check functions are derived directly from the structure and annotations of the Experience graph, potentially incorporating information learned during the Summary or verification phase. They typically verify:

\begin{itemize}
    \item \textbf{Control Flow Conformance:} Does the Experience graph contain an outgoing edge from the node corresponding to $S_{\text{current}}$ labeled with action $A$? This ensures the action is sequentially valid.
    \item \textbf{State Preconditions:} Are any preconditions associated with the edge in the Experience met in $S_{\text{current}}$? (e.g., if the Experience requires a specific file to be open before an 'edit' action, the check function verifies this). These preconditions might be explicitly learned or implicitly derived from the context of the original traces.
    \item \textbf{Data/Parameter Constraints:} If the action $A$ involves parameters, are these parameters consistent with constraints specified in the Experience? (e.g., ensuring a numerical parameter stays within a range observed in safe traces).
    \item \textbf{Safety Invariants:} Check functions can enforce safety invariants identified during Summary or specified manually. This addresses the requirement that variable parts of an Experience should not compromise safety. For example, if generalization introduced a loop, a check function might enforce a maximum iteration count derived from safe traces.
    \item \textbf{Human Action Bypass:} If the sequence of actions being replayed exactly matches a segment of a raw, recorded human trace (the ground truth), the check function might be simplified. In this case, the check could potentially reduce to verifying the match against the trusted trace, effectively bypassing more complex state or invariant checks for that specific step, under the assumption that direct human actions are inherently safe within that context.
\end{itemize}

\subsection{Safety Guarantees and Formalism}

By ensuring that every procedural action taken by the agent during Replay passes the associated check functions, EFI provides a guarantee that the agent's execution trajectory conforms to the structure defined by the selected, known-safe Experience. This prevents the agent from deviating into unexpected or unverified procedural paths.

This enforcement mechanism can be related to formal concepts:

\begin{itemize}
    \item \textbf{Reference Monitor:} EFI acts as a reference monitor, where the Experience serves as the policy, agent actions are the monitored accesses, and the check functions implement the monitor response logic. It aims to satisfy complete mediation (all procedural actions are checked) and tamperproofness (assuming the EBAE framework itself is secure).
    \item \textbf{Security Automata:} The Experience graph can be viewed as defining the structure of a security automaton. The automaton accepts only those sequences of actions (traces) that correspond to valid paths in the graph. The EFI check functions implement the automaton's transition logic, ensuring the agent's execution trace remains within the accepted language of the automaton.
    \item \textbf{Model Checking:} Conceptually, EFI performs a runtime model check at each step. The Experience is the model, the desired property is "adherence to the model's allowed transitions," and the check function verifies this property for the agent's proposed next action in the current state.
\end{itemize}

\textbf{Limitations:} The safety guarantee provided by EFI applies only to the procedural aspects (the edges) of the execution. It does not constrain the agent's behavior within creative nodes. The overall safety also depends critically on the correctness and safety-preserving nature of the Record and Summary phases – EFI can only enforce the safety encoded within the Experience it is given. If the Experience itself is flawed or unsafe due to errors in recording or generalization, EFI will enforce that flawed behavior.


==> impl.tex <==
\section{Implementation}

To demonstrate the feasibility of Experience-Based Agent Execution, we developed a prototype system. This section details its architecture and key implementation choices for each phase.

\subsection{Prototype System Architecture}

The EBAE prototype consists of several interconnected components, illustrated conceptually below:

\textbf{Recorder:} A background service responsible for capturing user actions. Our prototype focuses on desktop environments.

\textbf{Trace Storage:} A simple file-based storage for recorded sequences of actions (traces).

\textbf{Summarizer:} An offline component that processes traces to generate Experience graphs.

\textbf{Experience Store:} A local directory acting as a database for storing and retrieving Experience graphs (represented as serialized JSON).

\textbf{Agent Core:} The central component containing:

\begin{itemize}
    \item \textbf{Replayer:} Manages task execution based on a selected Experience.
    \item \textbf{LLM Interface:} Invokes a pre-trained LLM (e.g., GPT-4) for creative node execution.
    \item \textbf{Integrity Monitor:} Implements EFI by evaluating check functions before procedural actions.
    \item \textbf{Auditor:} Logs replay events to a file.
\end{itemize}

\textbf{Target Systems:} The applications (e.g., web browser, text editor, file explorer) the agent interacts with.

\subsection{Recording Mechanism}

Capturing user actions reliably across applications is challenging. Our prototype employs a combination of platform-specific APIs:

\textbf{Windows:} We utilize the Windows UI Automation (UIA) framework. Event handlers are registered to listen for specific UI events (e.g., button clicks, focus changes, text input changes) across applications. When an event occurs, UIA provides information about the source element (e.g., Name, AutomationId, ControlType) and the application process. This allows us to log semantic actions like \texttt{Click(button\_id)} or \texttt{Type(textbox\_id, text)}. We use helper functions similar to those found in automation tools to capture element details.

\textbf{Web Browser (Chrome):} A dedicated browser extension was developed. It uses standard WebExtension APIs to listen for DOM events (clicks, input changes), navigation events, and potentially intercepts network requests. It captures details like CSS selectors or element IDs for interacted elements. Communication between the extension and the main Recorder service allows integrating web actions into the overall trace. The Chrome DevTools Recorder API provides inspiration for capturing replayable actions.

\textbf{Correlation:} Events from different sources (UIA, browser extension) are correlated into a single trace based on timestamps and the currently focused application window.

\textbf{Challenges \& Simplifications:} The prototype focuses on single-threaded, sequential user actions. Mapping low-level events (e.g., raw key presses) to semantic actions requires heuristics (e.g., grouping key presses into Type events). Robustness to minor UI changes (e.g., button text modification) is limited in the current recorder; the Summarizer aims to mitigate this through abstraction. Privacy-sensitive data (e.g., passwords) are heuristically identified and masked in the trace. More advanced techniques like system-wide hooking or eBPF were considered but deemed too complex for the initial prototype, though they remain interesting avenues for future work to achieve more comprehensive recording.

\subsection{Summarization Algorithm}

The Summarizer transforms raw traces into Experience graphs.

\textbf{Algorithm Choice:} We implemented a summarization algorithm based on principles from process mining. Specifically, we first abstract the raw action trace into a sequence of higher-level activities (e.g., \texttt{Click(LoginButton)}, \texttt{Open(Document)}, \texttt{Call(SearchAPI)}). Then, we apply an inductive mining algorithm to discover a block-structured workflow model (represented as a Petri net variant) from one or multiple such activity sequences for the same task type. This approach handles sequences, choices, and loops.

\textbf{State Abstraction:} Nodes in the generated graph represent abstract states inferred by the miner based on activity dependencies, rather than concrete UI snapshots. Edges represent the procedural activities.

\textbf{Safety Considerations:} Generalization is currently based on the structure inferred by the miner. To enhance safety, we implemented constraints during mining: (1) Loops inferred must have a maximum iteration count derived from the longest observed loop instance in the traces. (2) Parameters within actions (e.g., specific URLs, file paths) are generalized using simple pattern matching or type abstraction, but the structure of the workflow itself is kept conservative, closely reflecting the observed traces. More advanced synthesis techniques focusing on verifiable output or post-mining verification are planned for future work. The current approach relies on the assumption that the observed human traces represent safe behavior and conservative generalization preserves this.

\subsection{Replay Engine}

The Replayer executes Experiences.

\textbf{Interaction:} It uses the same platform APIs as the Recorder (UIA, browser extension messaging) to interact with target applications, simulating clicks, typing, etc.

\textbf{Experience Traversal:} The Replayer maintains a pointer to the current node in the Experience graph. It identifies enabled procedural edges (actions) originating from the current node.

\textbf{Integrity Check:} Before executing an action $A$ corresponding to an edge, it calls the Integrity Monitor with the current state context and the proposed action $A$.

\textbf{Execution:} If the check passes, the Replayer executes the action using the appropriate API. Upon successful completion, it updates its current state based on the target node of the executed edge in the Experience graph.

\textbf{Creative Nodes:} When the current node is designated as creative, the Replayer formulates a prompt based on the task goal and current context (e.g., content of an open document) and sends it to the configured LLM API. The LLM response (e.g., generated text) is then inserted into the target application (e.g., typed into the editor) via the interaction APIs. The agent then transitions according to the Experience graph (potentially waiting for a user cue or a specific condition met by the LLM output).

\textbf{Error Handling:} Basic error handling is implemented (e.g., UI element not found, action failed). Currently, replay halts on error, logging the issue. More sophisticated recovery mechanisms are future work.

\subsection{Integrity Enforcement}

The Integrity Monitor is tightly integrated with the Replayer.

\textbf{Implementation:} It loads the selected Experience graph. When queried by the Replayer with a proposed action $A$ and current context $S_{\text{current}}$, it performs the checks described in Section 5.3:

\begin{itemize}
    \item It verifies that an edge corresponding to $A$ exists from the current node in the graph.
    \item It checks any simple preconditions associated with the edge (e.g., required application focus).
    \item It validates parameters against learned constraints (e.g., loop counters).
\end{itemize}

\textbf{Mechanism:} The checks are implemented as simple predicate functions operating on the graph structure and basic context information. Formal verification of the Experience itself is not yet implemented. The monitor returns a boolean allow/deny decision to the Replayer.

\subsection{Experience Store Implementation}

The prototype uses a simple file system-based Experience Store.

\textbf{Format:} Experience graphs are serialized to JSON files. Metadata (task name, creation date) is stored in the filename or a separate index file.

\textbf{API:} Basic functions allow listing available Experiences, loading an Experience by name, and saving a newly summarized Experience. Rating and auditing features are not implemented in the prototype.



\iffalse
This section provides a detailed description of the implementation of the Experience-based Agent Behavior Control method. The implementation focuses on the key components: Record \& Replay mechanisms, Experience Store, Execution Flow Integrity, and Graph Representation.

\subsection{Record Mechanism}
The Record mechanism captures user actions and stores them as traces. These traces are recorded using efficient data structures that allow for quick storage and retrieval. Algorithms are employed to ensure that the recording process is seamless and does not interfere with user activities.

\subsection{Replay Mechanism}
The Replay mechanism utilizes the recorded traces to guide agent actions. It employs algorithms that ensure agent actions align with user expectations and previously executed tasks. The Replay process is designed to be flexible, allowing for innovation within the content of tasks while maintaining procedural integrity.

\subsection{Experience Store}
The Experience Store is implemented as a database that stores and manages user experiences. Experiences are summarized and generalized using data management strategies that ensure efficient storage and retrieval. The system allows for the sharing and comparison of experiences, enhancing the agent's ability to adapt to different tasks and environments.

\subsection{Execution Flow Integrity}
Check functions are implemented to validate actions before execution, ensuring the integrity of the execution flow. These functions are integrated into the system to prevent unintended actions and maintain predictable and safe agent behavior.

\subsection{Graph Representation}
Agent behavior is represented as a state transition graph, implemented using algorithms that merge similar states and actions to create a generalized trajectory. This representation enhances the system's ability to adapt to different scenarios while maintaining safety and predictability.

\subsection{Technical Challenges and Solutions}
During the implementation, several technical challenges were encountered, including ensuring the efficiency of the Record \& Replay mechanisms and managing the complexity of the Experience Store. Solutions were developed to address these challenges, such as optimizing data structures and algorithms to improve performance and scalability. 
\fi

\iffalse
\begin{verbatim}
+-----------------+      +-----------------+      +-------------------+
| User Interface |----->| Recorder |----->| Trace Storage |
| (Applications) | | (UI Hooks, Ext) | | (Files/DB) |
+-----------------+      +-----------------+      +-------------------+
| |
| Records | Traces
                                  v                      v
+-----------------+      +-----------------+      +-------------------+
| Experience Store|<-+---| Summarizer |<-----+ |
| (DB/API) | | | (Proc. Mining / | | |
+-----------------+ | | Synthesis) | | |
        ^ | +-----------------+ | User Auditing/ |
| Selects | | Verification Loop |
| Experience | Experiences                +-------------------+
| |
+-------+---------+ | Uploads Experience
| Agent Core |--+
| (LLM + Replayer)|
| +---------------+ |
| | Integrity Mon.| |
| +---------------+ |
| +---------------+ |
| | Auditor | |
| +---------------+ |
+--------+--------+
| Executes Actions
| via OS/App APIs
         v
+-----------------+
| Target Systems |
| (Apps, Browser) |
+-----------------+
\end{verbatim}
\fi


==> relat.tex <==
\section{Related Works}

This section reviews existing literature on agent behavior control and related topics, providing context for the proposed Experience-based Agent Behavior Control method.

\subsection{Agent Behavior Control}
Existing methods for controlling agent behavior include rule-based systems, reinforcement learning, and supervised learning approaches. These methods often struggle to balance flexibility and control, with rule-based systems being too rigid and learning-based approaches lacking predictability. The proposed method addresses these challenges by using user behavior as a baseline, ensuring predictable and user-aligned actions.

\subsection{Large Model Hallucinations}
The hallucination problem in large models is a well-documented issue, with research focusing on understanding and mitigating its effects. Solutions often involve fine-tuning models or incorporating additional constraints. The proposed method mitigates hallucinations by constraining agent actions to those previously executed by users, reducing the risk of unpredictable behavior.

\subsection{User Behavior as a Baseline}
Research on using user behavior as a guiding framework for agent actions is limited but growing. Some approaches leverage user feedback or historical data to inform agent decisions. The proposed method extends this concept by using Record \& Replay mechanisms to ensure that agent actions align with user expectations and previously executed tasks.

\subsection{Record \& Replay Mechanisms}
Record \& Replay mechanisms are commonly used in software testing and debugging to reproduce and analyze system behavior. Their application to agent behavior control is novel, providing a structured way to guide agent actions based on user behavior. This approach enhances predictability and safety in agent operations.

\subsection{Summary}
In summary, while existing methods for agent behavior control offer valuable insights, they often fall short in balancing flexibility and control. The proposed Experience-based Agent Behavior Control method addresses these limitations by leveraging user behavior as a baseline, providing a novel and effective solution for controlling agent actions. 
